Temperley-Lieb Algebra: From Knot Theory to Logic and Computation via Quantum Mechanics

Our aim in this paper is to trace some of the surprising and beautiful connections which are beginning to emerge between a number of apparently disparate topics: Knot Theory, Categorical Quantum Mechanics, and Logic and Computation. We shall focus in particular on the following two topics: - The Temperley-Lieb algebra has always hitherto been presented as a quotient of some sort: either algebraically by generators and relations as in Jones' original presentation, or as a diagram algebra modulo planar isotopy as in Kauffman's presentation. We shall use tools from Geometry of Interaction, a dynamical interpretation of proofs under Cut Elimination developed as an off-shoot of Linear Logic, to give a direct description of the Temperley-Lieb category -- a "fully abstract presentation", in Computer Science terminology. This also brings something new to the Geometry of Interaction, since we are led to develop a planar version of it, and to verify that the interpretation of Cut-Elimination (the "Execution Formula", or "composition by feedback") preserves planarity. - We shall also show how the Temperley-Lieb algebra provides a natural setting in which computation can be performed diagrammatically as geometric simplification -- "yanking lines straight". We shall introduce a "planar lambda-calculus" for this purpose, and show how it can be interpreted in the Temperley-Lieb category.

==> pictures/PL1exap <==
.PS 0 1.25
circlerad = 0.05
A1: circle invis "$\cdots$"
A2: circle fill with .w at A1.e + (0.5,0)
A3: circle fill with .w at A2.e + (0.5,0)
A4: circle fill with .w at A3.e + (0.5,0)
B1: circle fill with .n at A1.s + (0, -2)
B2: circle invis "$\cdots$" with .w at B1.e + (0.5,0)
"$i$" at A2.n above
"$j$" at A3.n above
"$f(i)$" at A4.n above
"$f(j)$" at B1.s below
line from A3.s to B1.n
arc from A2.s to A4.s rad 0.5
.PE


==> pictures/PL2exp <==
.PS 0 1
circlerad = 0.05
A0: circle invis "$\cdots$" 
A1: circle fill with .w at A0.e + (0.5,0)
A2: circle invis "$\cdots$" with .w at A1.e + (0.5,0)
A3: circle fill with .w at A2.e + (0.5,0)
B1: circle fill with .n at A0.s + (0, -2)
B2: circle invis "$\cdots$" with .w at B1.e + (0.5,0)
B3: circle fill with .w at B2.e + (0.5,0)
"$i$" at A1.n above
"$j$" at A3.n above
"$f(j)$" at B1.s below
"$f(i)$" at B3.s below
line from A1.s to B3.n
line from A3.s to B1.n
.PE


==> pictures/TLidp <==
.PS 0 1
circlerad = 0.05
A1: circle fill
A2: circle fill with .w at A1.e + (0.5,0)
A3: circle invis "$\cdots$" with .w at A2.e + (0.5,0)
A4: circle fill with .w at A3.e + (0.5,0)
B1: circle fill with .n at A1.s + (0, -2)
B2: circle fill with .w at B1.e + (0.5,0)
B3: circle invis "$\cdots$" with .w at B2.e + (0.5,0)
B4: circle fill with .w at B3.e + (0.5,0)
"$1$" at A1.n above
"$2$" at A2.n above
"$n$" at A4.n above
"$1'$" at B1.s below
"$2'$" at B2.s below
"$n'$" at B4.s below
line from A1.s to B1.n
line from A2.s to B2.n
line from A4.s to B4.n
.PE


==> pictures/TLrel123p <==
.PS 0 1
circlerad = 0.05
linethick = 1
A1: circle fill
A2: circle fill with .w at A1.e + (0.5,0)
A3: circle fill with .w at A2.e + (0.5,0)
B1: circle fill with .n at A1.s + (0, -1)
B2: circle fill with .w at B1.e + (0.5,0)
B3: circle fill with .w at B2.e + (0.5,0)
C1: circle fill with .n at B1.s + (0, -1)
C2: circle fill with .w at C1.e + (0.5,0)
C3: circle fill with .w at C2.e + (0.5,0)
D1: circle fill with .n at C1.s + (0, -1)
D2: circle fill with .w at D1.e + (0.5,0)
D3: circle fill with .w at D2.e + (0.5,0)
arc from A1.s to A2.s rad 0.3
line from A3.s to B3.n
arc cw from B1.n to B2.n rad 0.3
line from B1.s to C1.n
arc from B2.s to B3.s rad 0.3
arc cw from C2.n to C3.n rad 0.3
arc from C1.s to C2.s rad 0.3
line from C3.s to D3.n
arc cw from D1.n to D2.n rad 0.3
"{\huge $=$}" at C3.e + (1.5, 0.5) 
E1: circle fill with .w at A3.e + (3, 0)
E2: circle fill with .w at E1.e + (0.5,0)
E3: circle fill with .w at E2.e + (0.5,0)
F1: circle fill with .w at D3.e + (3, 0)
F2: circle fill with .w at F1.e + (0.5,0)
F3: circle fill with .w at F2.e + (0.5,0)
arc from E1.s to E2.s rad 0.3
line from E3.s to F3.n
arc cw from F1.n to F2.n rad 0.3
"$U_{1}U_{2}U_{1} = U_{1}$" at D3.s + (1.5,-1.5)
A1: circle fill with .w at E3.e + (4, 0)
A2: circle fill with .w at A1.e + (0.5,0)
A3: circle fill with .w at A2.e + (0.5,0)
B1: circle fill with .n at A1.s + (0, -1)
B2: circle fill with .w at B1.e + (0.5,0)
B3: circle fill with .w at B2.e + (0.5,0)
C1: circle fill with .n at B1.s + (0, -1)
C2: circle fill with .w at C1.e + (0.5,0)
C3: circle fill with .w at C2.e + (0.5,0)
arc from A1.s to A2.s rad 0.3
line from A3.s to B3.n
arc cw from B1.n to B2.n rad 0.3
arc from B1.s to B2.s rad 0.3
line from B3.s to C3.n
arc cw from C1.n to C2.n rad 0.3
"{\huge $=$}" at B3.e + (2, 0) 
E1: circle fill with .w at A3.e + (4, 0)
E2: circle fill with .w at E1.e + (0.5,0)
E3: circle fill with .w at E2.e + (0.5,0)
F1: circle fill with .w at C3.e + (4, 0)
F2: circle fill with .w at F1.e + (0.5,0)
F3: circle fill with .w at F2.e + (0.5,0)
arc from E1.s to E2.s rad 0.3
line from E3.s to F3.n
arc cw from F1.n to F2.n rad 0.3
circle rad 0.25 with .c at B3.e + (3.5, 0)
"$U_{1}^2 = \delta U_{1}$" at C3.s + (2,-2.5)
A1: circle fill with .w at E3.e + (4, 0)
A2: circle fill with .w at A1.e + (0.5,0)
A3: circle fill with .w at A2.e + (0.5,0)
A4: circle fill with .w at A3.e + (0.5,0)
B1: circle fill with .n at A1.s + (0, -1)
B2: circle fill with .w at B1.e + (0.5,0)
B3: circle fill with .w at B2.e + (0.5,0)
B4: circle fill with .w at B3.e + (0.5,0)
C1: circle fill with .n at B1.s + (0, -1)
C2: circle fill with .w at C1.e + (0.5,0)
C3: circle fill with .w at C2.e + (0.5,0)
C4: circle fill with .w at C3.e + (0.5,0)
arc from A1.s to A2.s rad 0.3
line from A3.s to B3.n
line from A4.s to B4.s
arc cw from B1.n to B2.n rad 0.3
arc from B3.s to B4.s rad 0.3
line from B1.s to C1.n
line from B2.s to C2.n
arc cw from C3.n to C4.n rad 0.3
"{\huge $=$}" at B4.e + (2, 0) 
D1: circle fill with .w at A4.e + (4, 0)
D2: circle fill with .w at D1.e + (0.5,0)
D3: circle fill with .w at D2.e + (0.5,0)
D4: circle fill with .w at D3.e + (0.5,0)
E1: circle fill with .w at B4.e + (4, 0)
E2: circle fill with .w at E1.e + (0.5,0)
E3: circle fill with .w at E2.e + (0.5,0)
E4: circle fill with .w at E3.e + (0.5,0)
F1: circle fill with .w at C4.e + (4, 0)
F2: circle fill with .w at F1.e + (0.5,0)
F3: circle fill with .w at F2.e + (0.5,0)
F4: circle fill with .w at F3.e + (0.5,0)
arc from D3.s to D4.s rad 0.3
line from D1.s to E1.n
line from D2.s to E2.n
arc cw from E3.n to E4.n rad 0.3
arc from E1.s to E2.s rad 0.3
line from E3.s to F3.n
line from E4.s to F4.n
arc cw from F1.n to F2.n rad 0.3
"$U_{1}U_{3} = U_{3} U_{1}$" at C4.s + (2,-2.5)
.PE


==> pictures/TLrel12p <==
.PS 0 1
circlerad = 0.05
linethick = 1
A1: circle fill
A2: circle fill with .w at A1.e + (0.5,0)
A3: circle fill with .w at A2.e + (0.5,0)
B1: circle fill with .n at A1.s + (0, -1)
B2: circle fill with .w at B1.e + (0.5,0)
B3: circle fill with .w at B2.e + (0.5,0)
C1: circle fill with .n at B1.s + (0, -1)
C2: circle fill with .w at C1.e + (0.5,0)
C3: circle fill with .w at C2.e + (0.5,0)
D1: circle fill with .n at C1.s + (0, -1)
D2: circle fill with .w at D1.e + (0.5,0)
D3: circle fill with .w at D2.e + (0.5,0)
arc from A1.s to A2.s rad 0.3
line from A3.s to B3.n
arc cw from B1.n to B2.n rad 0.3
line from B1.s to C1.n
arc from B2.s to B3.s rad 0.3
arc cw from C2.n to C3.n rad 0.3
arc from C1.s to C2.s rad 0.3
line from C3.s to D3.n
arc cw from D1.n to D2.n rad 0.3
"{\huge $=$}" at C3.e + (1.5, 0.5) 
E1: circle fill with .w at A3.e + (3, 0)
E2: circle fill with .w at E1.e + (0.5,0)
E3: circle fill with .w at E2.e + (0.5,0)
F1: circle fill with .w at D3.e + (3, 0)
F2: circle fill with .w at F1.e + (0.5,0)
F3: circle fill with .w at F2.e + (0.5,0)
arc from E1.s to E2.s rad 0.3
line from E3.s to F3.n
arc cw from F1.n to F2.n rad 0.3
"$U_{1}U_{2}U_{1} = U_{1}$" at D3.s + (1.5,-1.5)
A1: circle fill with .w at E3.e + (4, 0)
A2: circle fill with .w at A1.e + (0.5,0)
A3: circle fill with .w at A2.e + (0.5,0)
B1: circle fill with .n at A1.s + (0, -1)
B2: circle fill with .w at B1.e + (0.5,0)
B3: circle fill with .w at B2.e + (0.5,0)
C1: circle fill with .n at B1.s + (0, -1)
C2: circle fill with .w at C1.e + (0.5,0)
C3: circle fill with .w at C2.e + (0.5,0)
arc from A1.s to A2.s rad 0.3
line from A3.s to B3.n
arc cw from B1.n to B2.n rad 0.3
arc from B1.s to B2.s rad 0.3
line from B3.s to C3.n
arc cw from C1.n to C2.n rad 0.3
"{\huge $=$}" at B3.e + (2, 0) 
E1: circle fill with .w at A3.e + (4, 0)
E2: circle fill with .w at E1.e + (0.5,0)
E3: circle fill with .w at E2.e + (0.5,0)
F1: circle fill with .w at C3.e + (4, 0)
F2: circle fill with .w at F1.e + (0.5,0)
F3: circle fill with .w at F2.e + (0.5,0)
arc from E1.s to E2.s rad 0.3
line from E3.s to F3.n
arc cw from F1.n to F2.n rad 0.3
circle rad 0.25 with .c at B3.e + (3.5, 0)
"$U_{1}^2 = \delta U_{1}$" at C3.s + (2,-2.5)
.PE


==> pictures/TLrel1p <==
.PS 0 1
circlerad = 0.05
linethick = 1
A1: circle fill
A2: circle fill with .w at A1.e + (0.5,0)
A3: circle fill with .w at A2.e + (0.5,0)
B1: circle fill with .n at A1.s + (0, -1)
B2: circle fill with .w at B1.e + (0.5,0)
B3: circle fill with .w at B2.e + (0.5,0)
C1: circle fill with .n at B1.s + (0, -1)
C2: circle fill with .w at C1.e + (0.5,0)
C3: circle fill with .w at C2.e + (0.5,0)
D1: circle fill with .n at C1.s + (0, -1)
D2: circle fill with .w at D1.e + (0.5,0)
D3: circle fill with .w at D2.e + (0.5,0)
arc from A1.s to A2.s rad 0.3
line from A3.s to B3.n
arc cw from B1.n to B2.n rad 0.3
line from B1.s to C1.n
arc from B2.s to B3.s rad 0.3
arc cw from C2.n to C3.n rad 0.3
arc from C1.s to C2.s rad 0.3
line from C3.s to D3.n
arc cw from D1.n to D2.n rad 0.3
"{\huge $=$}" at C3.e + (1.5, 0.5) 
E1: circle fill with .w at A3.e + (3, 0)
E2: circle fill with .w at E1.e + (0.5,0)
E3: circle fill with .w at E2.e + (0.5,0)
F1: circle fill with .w at D3.e + (3, 0)
F2: circle fill with .w at F1.e + (0.5,0)
F3: circle fill with .w at F2.e + (0.5,0)
arc from E1.s to E2.s rad 0.3
line from E3.s to F3.n
arc cw from F1.n to F2.n rad 0.3
.PE


==> pictures/TLrel2p <==
.PS 0 1
circlerad = 0.05
linethick = 1
A1: circle fill
A2: circle fill with .w at A1.e + (0.5,0)
A3: circle fill with .w at A2.e + (0.5,0)
B1: circle fill with .n at A1.s + (0, -1)
B2: circle fill with .w at B1.e + (0.5,0)
B3: circle fill with .w at B2.e + (0.5,0)
C1: circle fill with .n at B1.s + (0, -1)
C2: circle fill with .w at C1.e + (0.5,0)
C3: circle fill with .w at C2.e + (0.5,0)
arc from A1.s to A2.s rad 0.3
line from A3.s to B3.n
arc cw from B1.n to B2.n rad 0.3
arc from B1.s to B2.s rad 0.3
line from B3.s to C3.n
arc cw from C1.n to C2.n rad 0.3
"{\huge $=$}" at B3.e + (2, 0) 
E1: circle fill with .w at A3.e + (4, 0)
E2: circle fill with .w at E1.e + (0.5,0)
E3: circle fill with .w at E2.e + (0.5,0)
F1: circle fill with .w at C3.e + (4, 0)
F2: circle fill with .w at F1.e + (0.5,0)
F3: circle fill with .w at F2.e + (0.5,0)
arc from E1.s to E2.s rad 0.3
line from E3.s to F3.n
arc cw from F1.n to F2.n rad 0.3
circle rad 0.25 with .c at B3.e + (3.5, 0)
.PE


==> pictures/TLrel3p <==
.PS 0 1
circlerad = 0.05
linethick = 1
A1: circle fill
A2: circle fill with .w at A1.e + (0.5,0)
A3: circle fill with .w at A2.e + (0.5,0)
A4: circle fill with .w at A3.e + (0.5,0)
B1: circle fill with .n at A1.s + (0, -1)
B2: circle fill with .w at B1.e + (0.5,0)
B3: circle fill with .w at B2.e + (0.5,0)
B4: circle fill with .w at B3.e + (0.5,0)
C1: circle fill with .n at B1.s + (0, -1)
C2: circle fill with .w at C1.e + (0.5,0)
C3: circle fill with .w at C2.e + (0.5,0)
C4: circle fill with .w at C3.e + (0.5,0)
arc from A1.s to A2.s rad 0.3
line from A3.s to B3.n
line from A4.s to B4.s
arc cw from B1.n to B2.n rad 0.3
arc from B3.s to B4.s rad 0.3
line from B1.s to C1.n
line from B2.s to C2.n
arc cw from C3.n to C4.n rad 0.3
"{\huge $=$}" at B4.e + (2, 0) 
D1: circle fill with .w at A4.e + (4, 0)
D2: circle fill with .w at D1.e + (0.5,0)
D3: circle fill with .w at D2.e + (0.5,0)
D4: circle fill with .w at D3.e + (0.5,0)
E1: circle fill with .w at B4.e + (4, 0)
E2: circle fill with .w at E1.e + (0.5,0)
E3: circle fill with .w at E2.e + (0.5,0)
E4: circle fill with .w at E3.e + (0.5,0)
F1: circle fill with .w at C4.e + (4, 0)
F2: circle fill with .w at F1.e + (0.5,0)
F3: circle fill with .w at F2.e + (0.5,0)
F4: circle fill with .w at F3.e + (0.5,0)
arc from D3.s to D4.s rad 0.3
line from D1.s to E1.n
line from D2.s to E2.n
arc cw from E3.n to E4.n rad 0.3
arc from E1.s to E2.s rad 0.3
line from E3.s to F3.n
line from E4.s to F4.n
arc cw from F1.n to F2.n rad 0.3
"$U_{1}U_{3} = U_{3} U_{1}$" at C4.s + (2,-2.5)
.PE

